PopALM: Popularity-Aligned Language Models for Social Media Trendy Response Prediction

Social media platforms are daily exhibiting millions of events. To preliminarily predict the mainstream public reaction to these events, we study trendy response prediction to automatically generate top-liked user replies to social media events. While previous works focus on generating responses without factoring in popularity, we propose Popularity-Aligned Language Models (PopALM) to distinguish responses liked by a larger audience through reinforcement learning. Recognizing the noisy labels from user "likes", we tailor-make curriculum learning in proximal policy optimization (PPO) to help models capture the essential samples for easy-to-hard training. In experiments, we build a large-scale Weibo dataset for trendy response prediction, and its results show that PopALM can help boost the performance of advanced language models.

==> tables/caseStudy_ch.tex <==

\begin{CJK}{UTF8}{gbsn} 
\begin{table*}[!ht] 
    \resizebox{\columnwidth*2}{!}{%
    \begin{tabular}{p{2\columnwidth}}
        \hline        
        {\bf Post}:
         \ \#哈工大通报志愿者拍考研试卷袋\#：其未接触到试卷拟邀上级部门调查。近日，哈尔滨工业大学
         一志愿者对研究生招生考试试卷袋拍照并发到网上，引发关注。经初步调查，该志愿者工作是在自命题空
         信封上粘贴条形码，全程不能接触到试卷。\\
         \hline

         {\bf ChatGPT:} \ 根据通报中的信息，该志愿者的工作只是在自命题空信封上粘贴条形码，没有接触到真正
         的试卷。学校进行了初步调查，并计划邀请上级部门进行进一步调查，这表明他们对此事件的重视程度。\\
         {\bf ChatGLM:} \ 这条微博的通报信息是准确的，志愿者在考试袋上粘贴条形码并拍照，因此可以排除志愿者
        与考试试卷的接触到的可能性。然而邀请进行上级部门的调查，这可能会引起公众的担忧。\\
         {\bf ChatGLM (P-T):} \ 志愿者是志愿者,考生是考生,都别骂了,这样很没意义。\\
         {\bf ChatGLM (PPO):} \ 别拿志愿者说事了。\\
        {\bf ChatGLM (CL-PPO):} 别搞这些有的没的,该处理处理,该处罚处罚,不要搞什么表面工作。  \\
        \hline
    \end{tabular}
    }
    \caption{The original Chinese content of the
case study.}  
\label{table:caseStudyCh}
\vspace{-5mm}
\end{table*}  
\end{CJK}








==> tables/error_analysis.tex <==
\begin{table}[!ht] 
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccccccc}
        \hline        
        {\bf Post}:
         \ \#He Junlin becomes an intern anchor at the Film Channel\#. \\
         \ Welcome! Looking forward to the debut performance of intern He!" \\
         \ \#HeJunlinHostsChineseFilmReport\#\\
        \hline
        {\bf PppALM Predict-1:}: Looking forward to Xiao He.\\
        {\bf PppALM Predict-2:}: Looking forward to XiaoHe's internship.\\
        {\bf PppALM Predict-3:}: Looking forward to Xiao He!\\
        \hline
    \end{tabular}
    }
    \caption{Error Analysis.}  
\vspace{-5mm}
\end{table}  









==> texFiles/discussion.tex <==
\section{Discussion}\label{sec:discussion}

% \paragraph{Noise Discussion.}
% 我们在文章中我们定义的noise是文本本身没有意义，like "hahaha"等，但是由于社交媒体用户的casual behavior，得到了很大的赞。 这些数据导致了我们的reward model 不能很好的辨别。我们的PopALM可以针对情况，利用三个模块来提高模型效果。
\paragraph{Noise Handling.}
Parts of noisy labels may come from the casual behavior of user likes, as we discussed in the introduction, user likes may exhibit some sort of randomness and exhibit implicit relations with the response content itself. In this paper, such noisy labels make it challenging for the reward model to distinguish whether a response is popular and reflects public voice. Our curriculum learning design (CL-PPO) allows learning from easy to hard, which enables better learning results from noisy labels. Other noise may come from a few popular users whose comments collect lots of likes no matter what they post. For this noise, when constructing our dataset, we directly collected comments from posts of the most popular hashtags without specifically recording author information. This approach ensures that the data collected is more general. However, at the same time, we haven't completely excluded the influence of these authors. Many popular users might also be opinion leaders, and often, they lead the mainstream voice on social media. Our model learning from them is beneficial for trendy response generation.


\paragraph{Potential Application.}
We study trendy response prediction to automate the generation of top-liked user responses, which can helpfully train language models to predict the mainstream public reaction before an event happens or in its early stages. It has many potential applications. For example, it can be applied in early event analysis to foresee the future impact of a breaking event before many people engage in related discussions. Also, social scientists can employ our model to simulate the public responses to some social events even though they have not yet happened. Moreover, our study can potentially benefit general comment generation applications \cite{autoCommentGen1,autoCommentGenAAAI,autoGenTOMM}, and encourage better user engagement.

==> texFiles/limitation.tex <==
\section*{Limitations}
Here, we describe the shortcomings of our model. On the one hand, we found that in many instances, PopALM would generate meaningless but common responses, such as ``Support ...'', ``hahahahaha'', ``Go for it.'' 
Our analysis indicates that such responses represent a significant proportion of the training data, and these types of responses receive a considerable number of likes, causing the reward model to assign high scores to these responses. Therefore, in future work, beyond considering the popularity of responses, we should take a step further to factor in the quality of responses.

On the other hand, for the aspect of automatic evaluation, even though our proposed CL-PPO shows a promising improvement over PPO, the increase is not substantial. Essentially, our method strengthens the process of data selection and learning sequence, which does not result in a qualitative leap in predicting trendy responses. Moreover, from the perspective of human evaluation, although our model can predict popularity, it loses informativeness in the process. Based on these two points, in future work, we plan to provide the model with some external knowledge. By doing this, we aim to ensure it can learn popularity effectively while aligning well with the post's theme.
